Design, construction and operation of the ProtoDUNE-SP Liquid Argon TPC

The ProtoDUNE-SP detector is a single-phase liquid argon time projection chamber (LArTPC) that was constructed and operated in the CERN North Area at the end of the H4 beamline. This detector is a prototype for the first far detector module of the Deep Underground Neutrino Experiment (DUNE), which will be constructed at the Sandford Underground Research Facility (SURF) in Lead, South Dakota, USA. The ProtoDUNE-SP detector incorporates full-size components as designed for DUNE and has an active volume of $7\times 6\times 7.2$~m$^3$. The H4 beam delivers incident particles with well-measured momenta and high-purity particle identification. ProtoDUNE-SP's successful operation between 2018 and 2020 demonstrates the effectiveness of the single-phase far detector design. This paper describes the design, construction, assembly and operation of the detector components.

==> files-to-edit/camera.tex <==
\subsection{Cameras}
\label{sec:ci:camera}

Cameras provide direct visual information about the state of the
detector during critical operations and when damage or unusual
conditions are suspected. Cameras can be used to verify stability, straightness, and alignment of the hanging TPC structures during cool-down and filling; ensure that no bubbling occurs near the Ground Planes; inspect the state of movable parts in the detector (dynamic temperature sensor).
Eleven cameras were deployed in \pdsp{} at the locations shown in Figure~\ref{fig:pdsp-camera-locations}. They successfully provided views of the detector during filling and throughout %the 
its operation. % of the detector.

\begin{figure}[ht]
\begin{center}

 \includegraphics[width=0.6\textwidth]{figures/fig-cryo-instrumentation/pdsp-camera-locations-3d.jpg}
\caption{A 3D view showing the locations of the 11 cameras in \pdsp{}.}.
\label{fig:pdsp-camera-locations}
\end{center}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Cryogenic Cameras (Cold)}

The fixed cameras
monitor the following items during filling:
\begin{itemize}
\item positions of corners of APA, \dword{cpa}, FC, GP (\SI{1}{mm} resolution);
\item relative straightness and alignment of APA, CPA, and FC %(\(\lesssim\SI{1}{mm}\))
(\lesssim\,1\,mm);
\item relative positions of profiles and endcaps (\SI{0.5}{mm} resolution); and 
\item the LAr surface, specifically, the presence of bubbling or debris.
\end{itemize}


One design for the \pdsp{} fixed cameras uses an enclosure similar to the successful EXO-100 design \cite{Delaquis:2013hva}, see Figure~\ref{fig:gen-fdgen-cameras-enclosure}. Cameras 101, 102, 104, and 105, shown in Figure~\ref{fig:pdsp-camera-locations}, use this enclosure.
A thermocouple in the enclosure allows temperature monitoring, and a heating element provides temperature control.  
SUB-D connectors are used at the cryostat flanges and the camera enclosure for signal, power, and control connections.

\begin{figure}[ht]
\begin{center}
  \includegraphics[width=0.4\textwidth]{figures/fig-cryo-instrumentation/exo100-camera-case.jpeg}%
  \includegraphics[width=0.4\textwidth]{figures/fig-cryo-instrumentation/edgar-cameras.jpg}\\
  \hfill \includegraphics[width=0.22\textwidth]{figures/fig-cryo-instrumentation/bo-camera.jpg}%
  \hfill \includegraphics[width=0.22\textwidth]{figures/fig-cryo-instrumentation/camera-105-purmon-orig-rot-crop.jpg}%
   \hfill
   \caption{Top left: a CAD exploded view of a vacuum-tight camera enclosure suitable for cryogenic applications \cite{Delaquis:2013hva}.
    (1) quartz window, (2 and 7) copper gasket, (3 and 6) flanges, (4) indium wires, (5) body piece, (8) signal \fdth.
    Top right: two of the \dword{pdsp} cameras using a stainless steel enclosure. 
    Bottom left: one of the \dword{pdsp} cameras using acrylic enclosure.
    Bottom right: a portion of an image taken with \dword{pdsp} camera 105 showing a purity monitor mounted outside the \dword{apa} on the beam left side. This photo was taken with \dword{pdsp} completely filled.
  }
  \label{fig:gen-fdgen-cameras-enclosure}
  \end{center}
\end{figure}

An alternative successful design uses an acrylic enclosure, see Figure~\ref{fig:gen-fdgen-cameras-enclosure}, bottom left. Cameras 001, 002, 004, and 005, shown in Figure~\ref{fig:pdsp-camera-locations}, use acrylic enclosures. 
All operate successfully, including those at the bottom of the cryostat.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\subsubsection{Inspection Cameras (Warm)}
The inspection cameras are intended to be as versatile as possible.
Following inspections have been done with the warm cameras:

\begin{itemize}
\item status of HV-feedthrough and cup,
\item status of FC profiles, endcaps (\SI{0.5}{mm} resolution),
\item vertical deployment of calibration sources,
\item status of thermometers, especially dynamic thermometers,
\item HV discharge, corona, or streamers on HV feedthrough, cup, or FC,
\item relative position of profiles and endcaps (\SI{0.5}{mm} resolution), and
\item sense wires at the top of outer wire planes in the APA (\SI{0.5}{mm} resolution).
\end{itemize}

Unlike the fixed cameras, the inspection cameras operate only as
long as any inspection; the cameras can be replaced in case of failure.  It
is also more practical to keep the cameras continuously warmer than
 \SI{-150}{\celsius} during deployment; this allows use of commercial cameras, e.g., cameras of the same model were used successfully to observe discharges
in LAr from \SI{120}{cm} away \cite{Auger:2015xlo}.


\begin{figure}[ht]
\begin{center}
\label{fig:gen-fdgen-cameras}
  \includegraphics[height=0.3\textheight]{figures/fig-cryo-instrumentation/cisc-pdsp-camera-tube.jpg}%
\caption{A photo of the \pdsp{} warm inspection camera acrylic tube, immediately before installation; the acrylic tube is sealed with an acrylic dome at the bottom and can be opened at the top.}
\end{center}
\end{figure}

In this design, the warm camera is contained inside a gas-tight acrylic tube inserted into the feedthrough, and the warm cameras can be removed for servicing or upgrade at any time. Figure~\ref{fig:gen-fdgen-cameras} shows an acrylic tube enclosure and camera immediately before deployment. 
These acrylic tube enclosures for removable cameras were deployed at the positions marked 201, 202, and 203 in Figure~\ref{fig:pdsp-camera-locations}; they operated successfully. Cameras with fisheye lenses were used in these tubes during initial operation.  One camera was removed without any evidence of contamination of the LAr. The other cameras were used during post-beam running.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Light-emitting system}
The light-emitting system uses LED to illuminate
the parts of the detector in the camera's field of view with selected
wavelengths (IR and visible) that cameras can detect.  Performance criteria for the light-emission system include the efficiency with which the cameras can detect the light and the need to avoid
adding heat to the cryostat. Very high-efficiency
LED help reduce heat generation; one \SI{750}{nm} LED \cite{lumileds-DS144-pdf} has a specification equivalent to
\SI{33}{\%} conversion of electrical input power to light.

LED are placed in a ring around the outside of each
camera, pointing in the same direction as the lens, to 
illuminate nearby parts of the detector within the camera's field of
view. Commercially available LED exist with
a range of angular spreads that can be matched to the needs of the
cameras without additional optics.

Additionally, chains of LED connected in series and driven with a
constant-current circuit are used for broad illumination, with each
LED paired in parallel with an opposite polarity LED and a resistor
(see Figure~\ref{fig:cisc-LED}).
This allows two different wavelengths of illumination using a single chain simply by changing the direction of the drive current, and allows continued use of an LED chain even if individual LED fail.

\begin{figure}[ht]
\begin{center}
    \label{fig:cisc-LED}
  \includegraphics[width=0.6\textwidth]{figures/fig-cryo-instrumentation/cisc_led.png}
  \caption{Example schematic for LED chain, allowing failure tolerance and two LED illumination spectra.}
\end{center}
\end{figure}




==> files-to-edit/puritymon.tex <==
\subsubsection{Purity Monitor}
\label{sec:ci:purity}


Achieving a long enough electron lifetime so that electrons can drift sufficient distances is a challenging aspect of LArTPCs. The electron (e-) lifetime in a LArTPC is inversely proportional to, and determined by, the electronegative impurity concentration in the LAr, making the LAr purity an essential concern for successful operation and physics reach of the detector. 
Electron loss due to electronegative impurities in a LArTPC can be parameterised as $N(t)=N(0)e^{-t/\tau}$, where $N(0)$ is the number of electrons generated by ionisation and not recombined with argon ions, $N(t)$ is the number of electrons after drift time $t$, and $\tau$ is the electron lifetime. 
\pdsp{} was designed to have the same 3.6\,m drift distance and 500~V/cm electric field as  planned for the DUNE-SP far detector modules. Given the drift velocity of approximately 1.5~mm/$\mathrm{\mu s}$ in this field, the drift time from cathode to anode is roughly 2.3~ms. 
Thus, if the electron lifetime is $\mathrm{2.3 ms}/[-\ln(0.8)] \simeq \mathrm{10~ms}$, then the LArTPC signal attenuation, \([N(0)-N(t)]/N(0)\), remains less than 20\% over the entire drift distance.

%The following subsections provide details about the purity monitors, temperature sensors, and cameras.

\begin{figure}
\begin{center}
\includegraphics[width=0.9\textwidth]{figures/fig-cryo-instrumentation/cisc_pdsp_instrumentation.png}
\caption{Top view of the cryostat with the distribution of LAr instrumentation devices. The upstream side of the detector where the beam enters the cryostat is on the left hand side of the image. \label{fig:inst_map}}
\end{center}
\end{figure}

% A challenging aspect of liquid argon TPCs is to make electrons drift over long distances in LAr.  The electron lifetime which is determined by the LAr purity is an essential concern for successful operation and physics reach. In a LArTPC, electron loss due to electronegative impurity can be parameterized as $N(t)=N(0)e^{-t/\tau}$, where $N(0)$ is the number of electrons generated by ionization, $N(t)$ is the number of electrons after drifttime $t$, and $\tau$ is the electron lifetime. 

% I moved the following higher up (anne)
%ProtoDUNE-SP has the same the 3.5-m drift distance as the DUNE single phase far detector module, and the electric field is 500~V/cm. Given the drift velocity of approximately 1.5~mm/$\mathrm{\mu s}$ in this field, the time to go from cathode to anode is roughly 2.3~ms. If the LArTPC signal attenuation, \([N(0)-N(t)]/N(0)\), remains less than 20\% over the entire drift distance, the corresponding electron lifetime is $\mathrm{2.3 ms}/[-\ln(0.8)] \simeq \mathrm{10~ms}$.

Purity monitors are used to independently infer the effective free electron lifetime in a LArTPC.  
It works by illuminating a photocathode with deep UV light to generate an electron current, then collects the drifted current at an anode a known distance away. Attenuation of the
current is related to the electron lifetime. In the \pdsp{} purity monitors the UV light is generated by an external Xenon light source and delivered by quartz fibres to the inside of the cryostat. The fraction of photoelectrons generated at the purity monitor cathode that arrives at the anode ($Q_A/Q_C$) after the drift time $t$ is a measure of the electron lifetime $\tau$: $Q_A/Q_C=e^{-t/\tau}$, where $Q_C$ is the combined charge of the electrons generated at the photocathode, $Q_A$ is the combined charge of the electrons collected by the anode after drift time $t$, and $\tau$ is the electron lifetime.
%A purity monitor is a small time projection chamber (TPC) used to infer independently the effective free electron lifetime in the LAr TPC.   It illuminates a photocathode with deep UV light to generate a known electron current, then collects the drifted current at an anode a known distance away. The UV light is delivered by quartz fibers from a Xeon light source to the inside of the LAr cryostat. The electron (e-) lifetime in LAr is inversely proportional to the electronegative impurity concentration. The fraction of photoelectrons generated at the purity monitor cathode that arrive at the anode ($Q_A/Q_C$) after the drift time $t$ is a measure of the electron lifetime $\tau$: $Q_A/Q_C=e^{-t/\tau}$, where $Q_C$ is the charge of electrons generated at the photocathode, $Q_A$ is the charge of electrons collected by the anode after drift time $t$, and $\tau$ is the electron lifetime. 

The purity monitors are placed inside the cryostat but outside of the TPC volume due to their size. 

Although \pdsp{} receives ample cosmic ray data to perform electron lifetime measurements, the purity monitor system was found to be essential for providing quick, reliable, real-time information. It enabled operators to catch purity-related changes caused by LAr recirculation issues in time to correct them.
%Although ProtoDUNE receives ample cosmic ray data to perform electron lifetime measurements, the purity monitor system was found to be essential for providing quick, reliable real-time monitoring of purity in the detector and to catch purity-related changes in time due to LAr recirculation issues.

In addition, since the purity monitors have much smaller volumes than the LArTPC, the measurements from this system are affected to a much smaller degree by the space charge caused by cosmic rays.
%%% Note: I changed the meaning here (Anne) - please check!!!
%In addition the purity monitor electron lifetime measurements are precise, since the purity monitors have much smaller volumes compared to the TPC. Thus, electron lifetime measurements from purity monitors are much less affected by the space charge caused by cosmic rays.

\subsubsection*{Purity Monitor Design}

The purity monitor design follows that of the monitors used in the ICARUS experiment~\cite{Amerio:2004ze,Adamowski_2014} (Figure~\ref{fig:prm}). It consists of a double-grid ion chamber with four parallel, circular electrodes: a disk holding a photocathode, two grid rings (one each in front of the anode and the cathode), and an anode disk. The cathode grid (labelled ``ground-grid'' in the figure) is held at ground potential. The cathode, anode grid, and anode can each be independently biased via modified vacuum-grade HV feedthroughs. The anode grid and the field-shaping rings are connected to the cathode grid by an internal chain of 50\,$\mathrm{M\Omega}$ resistors to ensure the uniformity of the electric field in the drift regions. A stainless steel mesh cylinder is used as a Faraday cage to isolate the purity monitor from external electrostatic background. 

%The purity monitor design follows that of the monitors used in the ICARUS experiment~\cite{Amerio:2004ze} (Figure~\ref{fig:prm}).  It consists of a double-grid ion chamber with four parallel, circular electrodes, a disk holding a photocathode, two grid rings (in front of anode and cathode), and an anode disk. The cathode grid is held at ground potential. The cathode, anode grid, and anode each can be independently biased via modified vacuum-grade HV feedthroughs. The anode grid and the field-shaping rings are connected to the cathode grid by an internal chain of 50~$\mathrm{M\Omega}$ resistors to ensure the uniformity of the E field in the drift regions. A stainless mesh cylinder is used as a Faraday cage to isolate the purity monitor from external electrostatic background. 

\begin{figure}[h]
\centering
\includegraphics[width=0.7\textwidth]{figures/fig-cryo-instrumentation/PrMon_prm.pdf}
\caption{Schematic diagram of the %basic 
purity monitor design \cite{Amerio:2004ze}.}
 \label{fig:prm}
\end{figure}

Low signal strength has limited the precision and measuring ranges of purity monitors in previous LArTPC experiments \cite{AMERIO2004329}. To boost the signal strength for use in \pdsp{}, UV light was delivered to each purity monitor by eight fibres and an 8-channel feedthrough, resulting in signal magnitudes six times larger than with a single fibre. This increase came without penalty in timing resolution. 
%The signal strength of a purity monitor was an issue that has limited the precision and measuring ranges of purity monitors in previous LArTPC experiments. To increase the signal strength in ProtoDUNE, eight fibres were used with an 8-channel feedthrough to deliver UV light for each purity monitor. Signal magnitudes were 6 times larger than with a single fiber without penalty in timing resolution, thereby solving the long-existing signal strength problem. 

%The electron drift time is a key indicator of the measurement range and precision of the purity monitors. \todo{This pgraph is confusing. Drift times measured in the detector indicate how precise the purity monitor is? Please clarify whole paragraph! (anne)} During the commissioning and beam test of \pdsp{} the purity monitors were operated with different high voltages to change electron drift time (within the monitor?) over a range from 150$\mathrm{\mu s}$ to 3~ms. (3 ms sounds like drift time in detector) This allowed purity monitor measurements of the electron drift time in a range of 35$\mathrm{\mu s}$ to above 10~ms. 

The electron drift time is a key indicator of the measurement range and precision of the purity monitor. The electron drift time depends on the cathode - anode distance and the applied voltage within the monitor. During the commissioning and beam phase of \pdsp{} the electron drift time within the detector varied from 150$\mathrm{\mu s}$ to 3\,ms. The purity monitors were operated at different high voltage settings that allowed to cover an electron drift time measurement range of 35$\mathrm{\mu s}$ to more than 10\,ms. The drifting electron lifetime exceeded 3\,ms during beam time. The beam ended on the 12th of November.
%\todo{Is this less confusing now? (francesca)}

%The electron drift time is a key factor of the measurement range and precision of purity monitors. During the commissioning and beam test of ProtoDUNE the purity monitors operated with different high voltages to change electron drift time, ranging from 150$\mathrm{\mu s}$ to 3~ms. This allowed purity monitor measurements of the electron drift time in a range of 35$\mathrm{\mu s}$ to above 10~ms.

\subsubsection*{Purity Monitor Data}
Three purity monitors were installed in \pdsp{} (one each at the top, middle, and bottom) to 
continuously monitor the LAr purity during all stages:  commissioning, beam test, and operation. Figures~\ref{fig:prm-qaqc} and~\ref{fig:prm-lifetime} show the anode-to-cathode signal ratios $Q_A/Q_C$ and the electron lifetime measured by each purity monitor from the commissioning stage, which started in September 2018, through the entire beam test, which ended in November 2018, and continuing through the non-beam operations, which ended in February 2020. The shaded bands represent uncertainties in the measurements. All $Q_A/Q_C$ are normalised to a drift time of 2.3\,ms.
%Three purity monitors (top, middle, and bottom) were implemented in ProtoDUNE-SP. The purity monitors continuously monitored the LAr purity during all commissioning, beam test and operation periods of the detector. Figure \ref{fig:prm-qaqc} and \ref{fig:prm-lifetime} show the anode-to-cathode signal ratios $Q_A/Q_C$ and the electron lifetime measured by each purity monitor. The data are taken from the commissioning period of ProtoDUNE-SP starting in September 2018, through the entire beam running period (ending in December 2018), through February 2020. The shaded bands represent uncertainties of the measurements. All $Q_A/Q_C$ are normalized to drift time equal to 2.3 ms.

Each electron-lifetime measurement by the purity monitors is based on the signal ratios $Q_A/Q_C$ from 200 UV flashes at the same location occurring within a 40 second window. These measurements, taken regularly, were able to indicate incipient circulation-related issues on a quick timescale, mitigating potentially serious consequences for the detector. They caught a filter saturation during LAr filling, recirculation pump outages; these incidents show as sudden dips in Figures~\ref{fig:prm-qaqc} and~\ref{fig:prm-lifetime}.
%Each purity monitor electron lifetime measurement is based on purity monitor anode-to-cathode signal ratios $Q_A/Q_C$ from 200 UV flashes within 40 seconds at the same location. The regular measurement of the LAr purity performed by the purity monitors served as fundamental low reaction time measurements of insurging circulation related issues: A filter saturation during LAr filling, recirculation pump outages, and problems with the cryostat-level gauges. The dips in Figure \ref{fig:prm-qaqc} and \ref{fig:prm-lifetime} show these sudden changes in purity caught by the purity monitors, mitigating potentially serious consequences for the data taking ability of the detector.

The measurement uncertainties in Figure~\ref{fig:prm-qaqc} include statistical and time-dependent fluctuations, and uncertainties in the baseline of the purity monitor signal waveform, cathode and anode RC constants, the grid shielding inefficiencies, and grid transparency. Other uncertainties such as signal rise time, electron drift time, are found to be small. The overall uncertainties in purity-monitor charge ratio measurement $\frac{\Delta(Q_A/Q_C)}{(Q_A/Q_C)}$ at 2.3\ms drift time for the top, middle, and bottom purity monitors are $1.9\%$, $2.2\%$, and $3.9\%$, respectively. 

Note that given $Q_A/Q_C=e^{-t/\tau}$, when $Q_A/Q_C=1$, the measured lifetime $\tau$ is infinity. As shown in \ref{fig:prm-lifetime}, when the LAr purity is stabilised after filtering, $Q_A/Q_C$ is close to one, which means that the electron loss (due to impurities) after drifting for 2.3\,ms is very small. The top and middle purity monitors measured the electron lifetime to be greater than 70\,ms, and the bottom monitor measured it as greater than 30\,ms. These measurements indicate that \pdsp{} exceeded the high LAr purity required by the DUNE far detector.
%Note $Q_A/Q_C=e^{-t/\tau}$, when $Q_A/Q_C=1$, the measured lifetime $\tau$ is infinity. As shown in \ref{fig:prm-lifetime}, when the liquid argon purity is stabilized after filtering, $Q_A/Q_C$ is close to one, which means that the electron loss (due to impurity) after 2.3 ms drifting is very small. The top and middle purity monitors measured the electron lifetime to be greater than 20 ms, and the bottom purity monitor measured the electron lifetime to be greater than 10 ms. The measured electron lifetimes indicate that ProtoDUNE-SP has achieved the high liquid argon purity that will be required by the  DUNE far detectors.

Again given  $Q_A/Q_C=e^{-t/\tau}$, the relative uncertainty in lifetime $\Delta\tau/\tau$ is propagated as $\Delta\tau/\tau=(\tau/t)\frac{\Delta(Q_A/Q_C)}{(Q_A/Q_C)}$. It follows then that for a given $Q_A/Q_C$ uncertainty of  $\frac{\Delta(Q_A/Q_C)}{(Q_A/Q_C)}$, the relative uncertainty in the measured electron lifetime is proportional to the electron lifetime $\tau$ and inversely proportional to the electron drift time $t$. For a long electron lifetime, the relative uncertainty in this lifetime is large, as shown in Figure~\ref{fig:prm-lifetime}. However, since the main sources of uncertainties in $Q_A/Q_C$ are not correlated with the lifetime, $\frac{\Delta(Q_A/Q_C)}{(Q_A/Q_C)}$ is not significantly correlated with the electron lifetime or the drift time, and therefore the large relative lifetime uncertainty at high purity does not indicate lower precision in the purity monitor's measurement of the charge loss during electron drift time.The run-by-run purity monitor electron lifetime has been included in the ProtoDUNE-SP calibration database for TPC charge and energy calibration. The performance of the purity monitor based electron lifetime calibration tested with ProtoDUNE-SP cosmic rays is shown in Figure~\ref{fig:PrMCosmic}~\cite{ref:prmcalibUser2020}. After the purity-monitor-based lifetime calibration, the LAr impurity caused charge loss on the TPC signal is mostly corrected.

%From  $Q_A/Q_C=e^{-t/\tau}$,  the relative uncertainty in lifetime $\Delta\tau/\tau$ is propagated as $\Delta\tau/\tau=(\tau/t)\frac{\Delta(Q_A/Q_C)}{(Q_A/Q_C)}$. Therefore, for a given $Q_A/Q_C$ uncertainty $\frac{\Delta(Q_A/Q_C)}{(Q_A/Q_C)}$, the relative uncertainty in the measured electron lifetime is proportional to electron lifetime $\tau$ and inversely proportional to the electron drift time $t$. When electron lifetime is high, the relative uncertainty in electron lifetime is large, as shown in Figure \ref{fig:prm-lifetime}. However, since the main sources of uncertainties in $Q_A/Q_C$ are not correlated to electron lifetime, $\frac{\Delta(Q_A/Q_C)}{(Q_A/Q_C)}$ is not significantly correlated with the electron lifetime and drift time. Thus, the large relative lifetime uncertainty at high purity does not mean that a purity monitor has a lower precision of the measurement of the charge loss during electron drifting.
\begin{figure}[h]
\centering
\includegraphics[width=1.0\textwidth]{figures/fig-cryo-instrumentation/QaQcAllCorMark.png}
\caption{
The anode-to-cathode signal ratios $Q_A/Q_C$ measured by three purity monitors in \pdsp{} as a function of time, September 2018 through February 2020. The purity is low prior to the start of circulation in October 2018. Later dips represent recirculation studies and recirculation pump stops. The shaded bands represent uncertainties of the measurements. }
%\textbf{\textcolor{red}}}
 \label{fig:prm-qaqc}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=1.0\textwidth]{figures/fig-cryo-instrumentation/LifetimeAllCorLogMark.png}
\caption{The electron lifetimes measured by three purity monitors in \pdsp{} as a function of time, September 2018 through February 2020. The purity is low prior to the start of circulation in October 2018. Later dips represent recirculation studies and recirculation pump stoppages. The shaded bands represent uncertainties of the measurements.} %\textbf{\textcolor{red}}}
 \label{fig:prm-lifetime}
\end{figure}


\begin{figure}[htbp]
\begin{center}
%\begin{minipage}[t]{10cm}

\includegraphics[width=1.0\textwidth]{figures/fig-cryo-instrumentation/PrMCosmic.png}
%\end{minipage}
\caption{Performance of the purity monitor based electron lifetime calibration for  cathode-crossing cosmic rays in ProtoDUNE-SP Phase-1: (Left) $dQ/dx$ distribution and (Right) $dQ/dx$ vs. electron drift distance $x$, comparing no calibration (green), space charge effect calibration (SCE) (blue), PrM electron lifetime calibration+SCE (violet), electron lifetime calibration+SCE+YZ correction, electron lifetime calibration+SCE+YZ+Y correction. After the purity monitor based lifetime calibration (violet), the 15\% charge loss on TPC signal (blue) is mostly corrected.} \label{fig:PrMCosmic}
\end{center}
\end{figure}



==> files-to-edit/t-pro_new.tex <==
\subsection{Temperature sensors}
\label{sec:ci:t-pro}

92 high-precision temperature sensors are used to monitor the inner cryostat volume for correct behaviour and to predict the electron lifetime in areas far from purity monitors, using CFD simulations.  
%A detailed 3D temperature map is important for monitoring the
%cryogenic system for correct functioning and the LAr for uniformity. Given the complexity and
%size of purity monitors, they can only be installed on the sides of the cryostat to provide a local
%measurement of LAr purity. A direct measurement of the LAr purity across the entire cryostat
%is not feasible, but a sufficiently detailed 3D temperature map based on CFD simulations can
%predict it. The vertical coordinate is especially important because it will relate closely to the LAr recirculation and uniformity.
They are distributed near the TPC walls in two ways (see Fig.~\ref{fig:cisc_t_map}):
i) forming two high density vertical arrays (called T-gradient monitors) and 
ii) in coarser 2D horizontal arrays %(called individual sensors) 
at the top and bottom of the TPC\footnote{bottom sensors were mounted on the LAr return pipes and top sensors on the ground planes}. 
%, where it is most crucial to know the temperature.
%Expected temperature variations inside the cryostat are very small (0.02K; see Figure 1.2), so
%sensors must be cross-calibrated to better than 0.005K. Most sensors will be calibrated in the
%laboratory before installation (installation is described in Section 1.4.5.2). Calibration before
%nstallation is the only option for sensors installed on the long sides of the detector and the top
%nd bottom of the cryostat, where space is limited. Given the precision required and the unknown
%ongevity of the sensors – possibly requiring another calibration after some time – an additional
%ethod will be used for T-gradient monitors installed on the short ends of the detector in the space
%etween the field cage end walls and the cryostat walls. There is sufficient space in this area for a
%ovable system, which can be used to cross calibrate the temperature sensors in situ, as described
%n 1.2.1.1.
Three elements are common to all systems: sensors, cables
and readout. Lake Shore PT102 platinum sensors with 100~$\Omega$ (at 0 °C) resistance were chosen based on previous experience from the 35t prototype\cite{}.
%because in the temperature range 83 K to 92 K they show high reproducibility of ∼ 5 mK and absolute temperature accuracy of 100 mK. 
For the inner readout cables, a custom
cable made by Axon was used. It consists of four AWG 28 teflon-jacketed copper wires, forming two twisted pairs, with a metallic external shield and an outer
teflon jacket ($\diameter$3.7 mm). The 4-wire measurement is crucial to eliminate influence of the resistance of the wires.
%Using a four-wire readout greatly reduces issues related to lead resistance, any parasitic resistances, connections through the flange, and general electromagnetic noise pick-up. 
Finally, the readout system 
%relies on a variant of an existing mass PT100 temperature readout system developed at CERN for one of the LHC experiments; prior  test and validation by the collaboration experts. The system 
consists in an electronic circuit which includes: 
i) a precise and accurate 1\,mA current source for the excitation of the sensors,  
ii) a multiplexing circuit connecting the temperature sensor signals and forwarding the selected one to a single line, 
iii) and a readout system based on National Instrument Compact RIO Device with a high accuracy voltage signal readout NI9238 module with 24 bits resolution over \SI{1}{V} range. 
%This device also drives the multiplexing circuit and performs the temperature value calculations. The Compact RIO device is connected to the Detector Ethernet Network sending the temperature values to the DCS software through the standard OPC UA driver.

% NOT SURE WE SHOULD INCLUDE THIS
% another set of 12 lower-precision sensors epoxied into the bottom membrane of the
% cryostat was used to monitor the cryostat filling in the initial stage.  Finally, the lateral wall  of  the  cryostat  was  equipped  with  5  sensors  to  monitor  the  temperature  during
% cooldown and filling.
%(“W” sensors in Fig.~\ref{fig:cisc_t_map}. 

Additionally, 12 standard temperature sensors are in contact with the bottom cryostat membrane to detect the presence of LAr when filling starts, and 5 standard sensors are epoxied into one of the lateral walls to measure the temperature of the cryostat  membrane at different heights during cool-down and filling.  


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Dynamic T-gradient monitor}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

This is the only movable system in \pdsp{}. 
%It was designed in response to the requirement for the 3-5\,mK measurement precision of the vertical temperature gradient over the full 7.5\,m height of the ProtoDUNE TPC due to less than 10\,mK expected variation. Dynamic T-gradient monitor successfully addressed this requirement with its ability to cross-calibrate all sensors in-situ, removing any uncertainty associated with sensors changing overtime or change in the environment with respect to sensor calibration done prior to installation in the detector. 
It is equipped with a stepper motor connected to a carrier rod, on which 24 temperature sensors are mounted. Spacing is 10 cm for five sensors at the top/bottom and 50 cm for the 14 sensors on the middle, being the first(last) sensor at 10(750) cm from the bottom membrane. Each sensor is soldered to a PCB. Cables are routed along the carrier rod and connected to flange with Sub-D connectors on both sides.

The carrier rod with sensors is contained inside the gas tight enclosure that can be seen in Fig.~\ref{fig:cisc_dynamic_T}-left.  The stepper motor is mounted on the outside of the enclosure and engages with the carrier rod via ferrofluidic dynamic seal and pinion and gear that converts rotational motion of the stepper motor to the linear motion of the rod without jeopardising the integrity of the argon atmosphere inside the enclosure. 

Stepper motor can move the rod up and down vertically, allowing measuring the temperature at various heights in the TPC, with adjacent sensors. In this way, assuming stable temperature profile over the calibration period of couple of minutes, any offset in the temperature readings between two sensors measuring temperature at the same TPC height, is attributed to the intrinsic offset between the two adjacent sensors, providing constants for their cross-calibration. By linking all adjacent sensors, it is possible to calibrate out all offsets with respect to a single temperature sensors and achieve precise measurement of the relative vertical T-gradient.
See Fig.~\ref{fig:cisc_dynamic_T}-right for the comparison of sensor readout before and after calibration. As it will be shown below (Sec.~\ref{sec:temp_analysis}), final confirmation of the robustness of the system was achieved during the pump off detector period when the temperature over the detector height becomes uniform. 
%The readings on the dynamic T-monitor were within 2-3/,mK after calibration constants were included, setting up the ultimate measurement precision of the system.

\begin{figure}[ht]
\begin{center}
%\includegraphics[width=0.48\textwidth]{figures/fig-cryo-instrumentation/cisc_dynamic_bottom_Sensors_prior.png}
%\includegraphics[width=0.48\textwidth]{figures/fig-cryo-instrumentation/cisc_dynamic_bottom_sensors_after.png}
\includegraphics[height=0.77\textwidth]{figures/fig-cryo-instrumentation/cisc_dynamic_enclosure.png}
\hspace{1cm}
\includegraphics[width=0.55\textwidth]{figures/fig-cryo-instrumentation/cisc_dynamic_bottom_sensors_before_after.png}
\caption{Left: Dynamic T-gradient monitor enclosure showing stepper motor on the side and viewports to visually check the motion of the system. The top part of the enclosure houses the carrier rod when the system moves up. Right: Temperature measurement by the 5 sensors closest to the cryostat floor before and after cross-calibration}.
\label{fig:cisc_dynamic_T}
\end{center}
\end{figure}

%The carrier rod with sensors is contained inside the gas tight enclosure that can be seen in Fig.~\ref{fig:cisc_dynamic_enclosure} along with the motor mounted on the outside. 
%The lowest sensor is placed 10\,cm from the bottom of the cryostat. While the bottom and top 5 sensors have 10\,cm spacing, the sensors in between, from 50\,cm to 750\,cm from the bottom rod tip are placed at 50\,cm spacing. 
%The spacing between the sensors has been determined based on expectation from the CFD simulations that predicted variation of less than couple of mK every 100\,cm. 

%\begin{figure}[ht]
%\begin{center}
%\includegraphics[height=0.51\textwidth]{figures/fig-cryo-instrumentation/cisc_dynamic_enclosure.png}

%\caption{Dynamic T-gradient monitor enclosure showing stepper motor on the side and viewports to visually check the motion of the system. The top part of the enclosure houses the carrier rod when the system moves up}.
%\label{fig:cisc_dynamic_enclosure}
%\end{center}
%\end{figure}



 


%The system is also equipped with several safety features. There are limit switches that limit the stepper motion within the enclosure and at safe distance from the cryostat floor. Limit on the maximum motor current to sense any obstruction to the rod movement. Finally motor can be engaged manually with a ranch in case of failure. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Static T-gradient monitor}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

A vertical array of 48 sensors was installed 20 cm away from the lateral field cage (see Fig.~\ref{fig:cisc_static_TG}-left). 
Spacing is 11.8 cm at the top/bottom and 23.6 cm for the 16 sensors on the middle, being the first(last) sensor at 30.2(738.5) cm from the bottom membrane. Mechanical rigidity is provided 
by a 80x25x3 $mm^3$ U-shaped fibreglass profile (FGP), which holds sensors and cables. Given the proximity to the field cage the entire system is surrounded by a Faraday cage made of nineteen 6 mm diameter stainless steel rods disposed vertically forming a cylinder of 12.5 cm diameter. Rods and FGP hung from the top and are  mechanically decoupled of each other to account for their different behaviour in cold. FR4 rings attached to the FGP are use to route the rods, keeping the cylindrical shape of the Faraday cage. 

Sensors are mounted on a 52x14 $mm^2$ PCB with an IDC-4 connector, such that they can be plugged-in at any time. Cables are housed in the inner part of the FGP and run vertically from the sensor to the flange, which has eight Sub-D 25-pins connectors. 

Sensors are cross-calibrated in the laboratory using a controlled environment. A calibration set consists of four sensors (one of them kept as reference for all sets) which are placed next to each other and submerged in LAr several times. The stability of the calibration system and the performance of the sensors and the readout system are shown in Fig.~\ref{fig:cisc_static_TG}-right. The accuracy of the calibration was estimated to be 2.6 mK \cite{Peris:2018}. 

\begin{figure}[ht]
\begin{center}
\includegraphics[height=0.45\textwidth]{figures/fig-cryo-instrumentation/cisc_static_photo.jpg}
\hspace{1cm}
\includegraphics[height=0.45\textwidth]{figures/fig-cryo-instrumentation/cisc_tsensor_calib.png}%
\caption{
Left: The Static T-Gradient monitor installed in \pdsp{}. 
 Right: Temperature offset between two sensors as a function of time for four independent immersions in LAr show the stability of the system.
 %The reproducibility of those sensors, defined as the RMS of the mean offset in the flat region, is $\sim \SI{1}{mK}$, The resolution for individual measurements, defined as the RMS of one of the offsets in the flat region, is better than \SI{0.5}{mK}. 
\label{fig:cisc_static_TG}}
\end{center}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Temperature data analysis}
\label{sec:temp_analysis}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% ~

%SAY SOMETHING ABOUT PUMPS-OFF

%Figure 1.7 shows the temperature profile measured by the dynamic T-Gradient monitor when the recirculation pumps are off. Under these conditions the temperature should be very homogeneous except near the surface. This is indeed what is observed in that figure, demonstrating the reliability of the calibration method based on the movable system. 
%This result is also used to prove the validity of a new calibration method, based on the assumption of homogeneous temperature when pumps are off. This method is used to cross-calibrate sensors in the Static T-Gradient monitor (see Fig.~\ref{}-right) and individual sensors. 

The systems described above have been collecting data for more than a year, resulting in a deeper general understanding of LAr dynamics inside cryostat. Some important facts have been proved and are being highlighted in the following.

Stability studies show that except near the LAr surface the difference in temperature between any two sensors in the same T-Gradient monitor remains constant within 3\,mK, probing the stability of the LAr regime for standard operating conditions, and the reliability/longevity of the sensors, which is one of the most significant results obtained. 

Dynamic T-Gradient monitor has been cross-calibrated several times. The obtained result is a smooth profile (see Fig.\ref{fig:protodune_general_performance_pumpoff}-left), as expected from a slow and continuous process in which sensors are progressively being place in each other's places. Any deviation from smoothness would have meant a bug in the device.

Vertical and horizontal profiles under several conditions (stable regime, with/without recirculating system, pressure changes) have been studied. The pumps-off (without recirculation) regime is particularly interesting since small temperature gradients are expected. This was observed by the Dynamic T-Gradient (see Fig.\ref{fig:protodune_general_performance_pumpoff}-left). The flatness of this profile points a big homogeneity of LAr temperature. This fact was used to re-calibrated the Static T-Gradient monitor (this is the so-called "pumps-off" calibration method) and the result compared to the laboratory calibration, showing good agreement (see Fig.\ref{fig:protodune_general_performance_pumpoff}-right). 

Those studies have also shown big differences in temperature when recirculating system is on or off. This differences were not originally expected and appear in vertical and horizontal planes. The grid of sensors placed 40 cm over cryostat bottom shows a temperate pick (20 mK) below the cathode plane and a decrease towards the pump when recirculating system is working (see Fig.~\ref{fig:protodune_general_performance_bottom}-left), and a more homogeneous distribution when it is not (see Fig.~\ref{fig:protodune_general_performance_bottom}-right).

Finally, Fig.~\ref{fig:protodune_general_performance_cfd_comparative} shows the comparison of the vertical profiles (stable regime) with CFD simulations for different boundary conditions (varying flow rate and temperature for the incoming LAr). The CFD model reasonably predicts the main features of the data but the details still need to be understood as the bump at 6.2 m and the lower measured temperature at the bottom. More studies on CFD boundary conditions are needed. 

\begin{figure}
\begin{center}
\includegraphics[width=0.98\textwidth]{figures/fig-cryo-instrumentation/cisc_t_bottom.png}
\caption{Temperature difference between Static T-Gradient bottom sensor and horizontal grid of sensors placed 40 over bottom membrane. Left and middle: temperature distribution when recirculating system is on. Right: temperature distribution when recirculating system if off.
\label{fig:protodune_general_performance_bottom}}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=0.49\textwidth]{figures/fig-cryo-instrumentation/protodune_general_performance_dynamic_flatness.pdf}
\includegraphics[width=0.49\textwidth]{figures/fig-cryo-instrumentation/protodune_general_performance_static_pumpoff.pdf}
\caption{Left: Dynamic T-Gradient with no recirculation shows a flat profile. Right: Static T-Gradient during gas pressure raising comparative between laboratory calibration and `pumps-off' calibration.
\label{fig:protodune_general_performance_pumpoff}}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=0.49\textwidth]{figures/fig-cryo-instrumentation/protodune_general_performance_static_fit.pdf}
\includegraphics[width=0.49\textwidth]{figures/fig-cryo-instrumentation/protodune_general_performance_dynamic_fit.pdf}
\caption{Temperature profiles measured by the T-gradient monitors and comparison to the CFD model with different boundary conditions. Left: Static T-gradient monitor; Right: Dynamic T-gradient monitor. Unless specified, LAr flow rate is nominal, 0.42kg/s.
\label{fig:protodune_general_performance_cfd_comparative}}
\end{center}
\end{figure}

